Pattern formation with pde2path -- a tutorial

We explain some pde2path setups for pattern formation in 1D, 2D and 3D. A focus is on new pde2path functions for branch switching at steady bifurcation points of higher multiplicity, typically due to discrete symmetries, but we also review general concepts of pattern formation and their handling in pde2path, including localized patterns and homoclinic snaking, again in 1D, 2D and 3D, based on the demo sh (Swift-Hohenberg equation). Next, the demos schnakpat (a Schnakenberg reaction-diffusion system) and chemtax (a quasilinear RD system with cross-diffusion from chemotaxis) simplify and unify previous results in a simple and concise way, CH (Cahn-Hilliard) deals with mass constraints, hexex deals with (multiple) branch points of higher degeneracy in a scalar problem on a hexagonal domain, and shgc illustrates some global coupling. The demos acS, actor, schnakS and schnaktor (the Allen-Cahn and Schnakenberg models on spheres and tori) consider pattern formation on curved surfaces, cpol considers a problem of cell polarization described by bulk-surface coupling, and bruosc (Brusselator) explains how to augment autonomous systems by a time periodic forcing. Along the way we also comment on the choice of meshes and mesh adaptation, on time integration, and we give some examples of branch point continuation and Hopf point continuation to approximate stability boundaries.

==> acsf1.tex <==
\begin{figure}[ht]
\bce 
\begin{tabular}{ll}
{\small (a) Real life}&{\small (b) $R=14$, BD of primary hex and stripes, 
and example plots}\\
\raisebox{25mm}{
\begin{tabular}{l}
\ig[width=0.18\textwidth]{pic/sS/radio1b}\\
\ig[width=0.18\textwidth]{pic/sS/phage1}
\end{tabular}}&
\hs{-1mm}\ig[width=0.2\textwidth]{pic/sS/bd14}
\hs{-2mm}\raisebox{25mm}{\begin{tabular}{ll}
\ig[width=0.18\textwidth]{pic/sS/14-1-25}
\raisebox{-3mm}{\ig[width=0.18\textwidth]{pic/sS/14-2-15}}\\
\ig[width=0.18\textwidth]{pic/sS/14-1-25S}
\ig[width=0.17\textwidth]{pic/sS/14-2-15S}
\end{tabular}}
\end{tabular}
\\
\begin{tabular}{ll}
{\small (c) $R=18$ }&{\small (d) plots from secondary branches }\\
\hs{-1mm}\ig[width=0.2\textwidth]{pic/sS/bd18}
\hs{-4mm}\raisebox{25mm}{\begin{tabular}{ll}
\ig[width=0.18\textwidth]{pic/sS/18-1-4-10}
\ig[width=0.18\textwidth]{pic/sS/18-2-1-20}\\
\ig[width=0.18\textwidth]{pic/sS/18-1-4-10S}
\ig[width=0.18\textwidth]{pic/sS/18-2-1-20S}
\end{tabular}}&
\raisebox{25mm}{\begin{tabular}{ll}
\ig[width=0.15\textwidth]{pic/sS/s1-8S}
\ig[width=0.15\textwidth]{pic/sS/s2-10S}\\
\ig[width=0.15\textwidth]{pic/sS/s5-10S}
\ig[width=0.15\textwidth]{pic/sS/s6-10S}
\end{tabular}}
\end{tabular}

\ece
\vs{-5mm}
   \caption{{\small Pattern formation on spheres. (a) Top: 
Silica skeletons of two radiolaria, scale about 1mm. 
Bottom: Two spherical virusses, scales about 100nm. All from \cite{VAB99}. (b)-(c) \reff{tur1b} on spheres  {\tt nt=10000} 
triangular elements. (b) $R=14$, stripes stable at large amplitude, and 
stable branch of two 'polar' hexagons. (c) $R=18$, stable hexagons 
(stability loss in fold). No stable stripes for $\lam>2.6$. 
(d) Some sketches of secondary bifurcations from stripes for illustration, 
all unstable. 
  \label{ssf1}}}
\end{figure}


==> fch.tex <==
\subsection{Pearling and meandering in the functionalized Cahn--Hilliard equation: Demo {\tt fCH}}\label{fchsec}
A binary mixture of a solvent (e.g.~water) and (hydrophobic) molecules 
(polymers or lipids) can be 'functionalized' by adding hydrophilic 
side chains to the molecules. Intuitely, this may favor the formation 
of bilayer interfaces (``channels'', see Fig.~\ref{fchf1}(a) for examples 
in the model given below), where the 
\ina{bilayer interface (channel)}
hydrophilic (hydrophobic) ends of the molecules 
point to the solvent (to the inside of the channel). In Fig.~\ref{fchf1},  
black corresponds to the low and yellow to a high concentration 
of molecules. 
If the mixture is dilute, the channels show a pearling instability, and if 
there is 'excess mass', i.e., 
a relatively high volume fraction of molecules, then channels tend 
to bend, which is also called meandering. 

The model we consider is from 
\cite{GJPY11, DHPW12}, to which we also refer for further background. 
Letting $u:\Om\to \R$ be the volume fraction of solvent and molecules, 
with $u=-1$ corresponding to pure solvent and 
some $u_+>0$ corresponding to saturation, 
the free energy of the mixture reads 
\huga{\label{fchE} 
\CF(u)=\int_\Om \frac 1 2 (\eps^2 \Delta u-W'(u))^2
-\eps^\beta\left(\frac{\eta_1} 2
\eps^2|\nabla u|^2+\eta_2W(u)\right)^2\dd x, 
}
where $0<\eps\ll 1$ is related to interface thickness, and $W:\R\to\R$ is 
a double--well potential with typically unequal strict 
minima at $-1$ and $u_+>0$, and a strict maximum at $u=0$. The first summand 
is the squared variational derivative of the Cahn--Hilliard energy $E_\eps(u)$, 
cf.~\reff{ch1}, and can thus be seen as a bending energy, also called 
Willmore functional. The second \ina{Willmore functional}
summand represents the functionalization, where $\eta_1>0$ and $\eta_2\in\R$ 
model the strenght of the hydrophilicity in terms of interfaces and volumes, 
respectively. Thus, $\eta_1>0$ means that interfaces lower the 
free energy. 

For $\beta=1$ ($\beta=2$) we have so called strong (weak) 
functionalization, and as in \cite{DHPW12} we focus on the strong case. 
The evolution of the system is assumed to be given by a \ina{gradient!operator}
gradient flow $\pa_t u=-\CG\del_u\CF(u)$, \ina{gradient!flow}
where 
the choice of the gradient operator $\CG$ together with the BCs must ensure 
mass conservation, i.e., $\ddt \int_\Om u(t,x)\dd x=0$. 
The simplest choice is the projection 
\huga{\label{fchg1}
\CG f=\Pi f:=f-\frac 1 {|\Om|}\int_\Om f(x)\dd x, 
}
leading to the evolution equation 
\huga{\label{tfch} 
\pa_t u=-\CG[(\eps^2\Del-W''(u)+\eps\eta_1)(\eps^2\Del u-W'(u))+\eps\eta_dW'(u)],
} 
where $\eta_d=\eta_2-\eta_1$. 
In suitable parameter regimes, \reff{tfch} 
is very rich in pattern formation. The basic building blocks (in 2D) 
are straight and curved  bilayer 
interfaces between $u\equiv -1$ and $u$ near $u_+$, which 
show ``pearling'' and ``meander'' instabilities as illustrated in 
Fig.~\ref{fchf1}(a). 

\taskip
\begin{table}[ht]\caption{Selected scripts and functions in {\tt pftut/fCH}. 
fchinits, oosetfemops, sG (with nodalf), and sGjac more or less as usual. 
\label{fchtab}}
{\small 
\begin{tabular}{l|p{0.81\textwidth}}
script/function&purpose,remarks\\
\hline
cmds1&script to continue a straight channel, and meandering and pearling 
bifurcations from it, Fig.~\ref{fchf1} \\
cmds2&script for continuation in $\eta_1$ and DNS, Fig.~\ref{fchf2}\\
e2rs\_ad\_hoc&trivial elements-to-refine-selector based on $|u+2|$\\
qf2, qf2jac&the phase conditions \reff{sfchs3} and \reff{fchpc}, and the derivatives\\
nodalft&modification of {\tt nodalf} (the 'nonlinear terms' in \reff{sfchs}), 
setting $\ga=0$ and including \reff{fchg1} for mass conservation. 
\end{tabular}
}
\end{table}
\teskip

A \pdep --setup for \reff{tfch} and some results were already presented 
in \cite{p2p2}, but without stability considerations. Moreover, 
here we present a simpler setup, and want to explain further tricks to 
compute patterns in \reff{tfch} more robustly. See Table \ref{fchtab} 
for an overview of the used files. 
Setting $v=\eps^2\Del u-W'(u)$, the problem can be written 
as the two component system 
\begin{subequations}\label{sfchs}
\hual{
\pa_t u=&-\eps^2 \Delta v+W''(u)v-\eps\eta_1 v-\eps\eta_dW'(u)+\eps\ga,\\
0=&-\eps^2 \Delta u+W'(u)+v,
}
where $\ga$ is the (scaled) Lagrange multiplier for mass conservation 
\ina{mass conservation}%
in \reff{tfch}, over domains $\Om$ with Neumann BCs for $u$ and $v$. 
We take $\ga$ as an additional unknown,  and add the equation 
\huga{\label{sfchs3}
q(u):=\frac 1 {|\Om|}\int_\Om u\dd x-m=0, 
}
\end{subequations}
where $m$ is a reference mass, also taken as a parameter, 
which here we shall use as the main continuation parameter 
as in the CH equation in \S\ref{chsec}.  
Moreover, as we shall be interested in rather dilute mixtures 
$m$ near $-1$, it turns out that often phase conditions are needed 
or at least very useful for robust continuation of patterns. 
For instance, for the channels in Fig.~\ref{fchf1} we use the 
phase condition 
\huga{\label{fchpc}
\spr{\sin(x),u}=\int_\Om \sin(x)u(x,t)\dd x=0, 
}
fixing the channel in the middle of the domain, and add $s\pa_x u$ 
to the rhs of (\ref{sfchs}a). 
Thus, we now have 4 parameters $(\eta_1,\eta_2,\eps,m)$, two 
additional unknowns $(\gamma,s)$, and two additional 
equations \reff{sfchs3} and \reff{fchpc}, i.e., $n_q=2$. 


For $W$ we follow \cite[\S5]{DHPW12} and let 
$$
W(u)=W_p(u+1)+20(u-m_p+1)^{p+1}H(u-m_p+1),\text{ where }
W_p(u)=\frac 1 {p-2}(pu^2-2u^p)
$$
with $p=3$, $m_p=(p/2)^{1/(p-2)}=3/2$, 
and $H$ being the Heaviside function. In \cite[\S5]{DHPW12}, additional 
to a strong analysis 
which establishes the existence of straight and curved channels and 
gives certain instability criteria for them, numerical 
time integrations are presented with $\eps=0.1$, 
$\eta_2=2$, and $\eta_1$ between 1 and 2. %(which leads to pearling), 
%resp.~$\eta_1=2$. %(which gives meandering). 
We use similar parameter 
regimes, but a somewhat larger $\eps=0.25$ to keep numerical costs low. 

\input{fchf1} 

Figure \ref{fchf1} shows a continuation of and bifurcation from 
a straight channel in the box $\Om=(-1,1)\times(-3,3)$, 
using $m$ as continuation parameter.  
The starting straight channel is obtained from the guess 
\huga{\label{fchiguess}
\text{$u_{ig}(x)=-1+a/\cosh(bx), \quad 
v_{ig}=-W'(u_{ig})$}}
with $a=1.25$, $b=20/3$, which yields the initial mass $m=m_0\approx -0.853$, 
followed by a Newton loop for \reff{sfchs}--\reff{fchpc}. 
It turns out that due to the large variety of patterns 
possible for \reff{sfchs}, a careful choice and refinement of meshes 
is important, 
in particular mesh symmetry. Thus, here we use a 
{\em very} ad--hoc refinement strategy, i.e., we replace 
the error estimator {\tt e2rs} by {\tt e2rs\_ad\_hoc}, 
which simply selects the triangles according $|u+2|$. 
For the initial guess \reff{fchiguess}, a 1--step mesh refinement 
from an initial criss--cross mesh of about 3500 points. 
then yields the first solution $u_0$ in Fig.~\ref{fchf1}(a), on a mesh 
of about 9000 points, refined around the $x=0$ line, and we keep 
this mesh for all the subsequent computations.%
\footnote{At the end of {\tt cmds2.m} we use \trulle\ 
to generate meshes which are clearly much better adapted to specific 
chosen solutions. However, using these meshes for continuation, 
with or without further adaptation during continuation, makes 
the continuation less robust: Often, genuine bifurcations on 
the symmetric mesh (which are also expected from theory) become 
imperfect bifurcations on the (anisotropic) \trulle\ meshes.} 

The straight channel solution $u_0$ at $m=m_0$ 
is unstable with $2$ unstable eigenvalues of $\pa_u G$ 
for \reff{sfchs} (which do not take into account the constraints 
\reff{sfchs3} and \reff{fchpc}), and for the time evolution 
of \reff{tfch}. 
These DNSs are again based on the formulation as the DAE system 
\reff{sfchs}, with both \reff{sfchs3} and the phase condition \reff{fchpc} 
switched off, and with $\ga=0$. We 
implement this by a small modifications of 
the library function {\tt tintxs} and of the 
nonlinearity function {\tt nodalf} used for \reff{sfchs}  
to account for $\Pi$ from \reff{fchg1}. 
Continuing $u_0$ to smaller $m$, we first find  two BPs BP1 and BP2 
at $m\approx -0.856$  and $m=-0.858$, respectively, 
after which the straight channel 
is stable until BP3 at $m\approx -0.868$, followed by 
BP4 at $m\approx -0.872$ and further BPs at lower $m$. 
BP1 and BP2 are associated to meandering, while BP3 and BP4 yield 
pearling, see (c) for the bifurcation directions, 
which illustrate the dichotomy between pearling 
at low $m$ (dilute mixture) and bending at 'high' $m$ (excess mass of 
the molecules).
The primary bifurcating meandering dark green branch {\tt m1} is stable after a 
fold. The primary blue pearling branch {\tt p1} bifurcates supercritically 
and is stable until $m\approx -0.9$ (secondary bifurcation not shown).  
Similar 
pearling branches bifurcate from the further BPs on the straight 
channel branch at lower $m$.   
Note that all these (pearling and meandering) 
bifurcations respect the (physical) 
constraint \reff{sfchs3}, and the numerical constraint \reff{fchpc}, 
which is needed for the continuation of the steady 
branches: omitting it, we get an eigenvalue very close to $0$ 
from shifting a solution in $x$, 
and relatedly we observe that some solutions drift during the 
continuation, even on the rather narrow domain, with the refined mesh 
near $x=0$. The pearling instabilities on the left only depend 
weakly on the transverse length $l_y$, as they are of relatively 
high wave number in $y$, but of course the bending may set in earlier on 
longer domains. 

\input{fchf2}

In \cite[Fig.5.1, Fig.5.2]{DHPW12}, an example is given where 
increasing $\eta_1$  yields pearling of a curved (circular) channel. 
To see this, in {\tt cmds2} and Fig.~\ref{fchf2}(a,b) we continue 
the meandering solution {\tt m1/pt10} in $\eta_1$. In 
Fig.~\ref{fchf2}(c) we show snapshots from a 
DNS starting near the unstable straight channel 
at $m=-0.8$ (with zero mass perturbation) 
which illustrates the typical behaviour at 'high' $m$ ($m>-0.82$, say). 
Initially, some (non--small wave number) pearling occurs, 
but most of the spots recombine to a curved channel, with a 
 pearled loop at the top. 
%which (located somewhere) 
%is  quite characteristic for all simulations of this kind.  
At $t=200$ the solution is already quite close to a steady state, i.e., 
the residual is below $10^{-8}$, and 
further DNS does not yield visible changes. Thus, we use  
this solution as initial guess for a Newton loop and obtain 
convergence to a steady state without visible change. Conversely, 
similar experiments at low $m$ 
(of course, the $m$ here also depends on the domain size in $x$, i.e., 
the same channels on domains twice as large in $x$ would yield $m$ values 
much closer to $-1$) typically yield convergence to straight pearled 
channels, i.e., no meandering at all. 

%\input{mod/fchf3}


\brem\label{fchrem}
The results in Fig.~\ref{fchf1} to Fig.~\ref{fchf2} only 
scratch the surface of a numerical exploration of the fCH equation 
\reff{tfch}, for which continuation is difficult due to the different 
length scales involved, and the many solutions supported. 
We further refer to \cite{CKP19} for remarkable 
DNS in 2D and 3D, which combined with analysis yield ``qualitative 
bifurcation diagrams'', which partition the parameter space into 
regions where pearling or meandering dominate. See also 
\cite{PW17} for modeling of biological systems (consisting of 
different lipids) by multi--component fCH systems. 
Nevertheless, we believe that numerical continuation and bifurcation 
as presented here may help to sort out the different parameter regimes 
more quantitatively. 
\eex\erem 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> psq.tex <==
\paragraph{$D_4$ symmetry on a non--square domain.} The double multiplicity 
of the BPs in Fig.~\ref{shf77b} and of many further BPs follows from 
$\Om$ being a square domain and the Neumann BCs. However, the 
generic form of the amplitude equations \reff{sqae} (in the case of a double BP) 
follows from the $D_4$ equivariance. Here we briefly discuss an example 
of the SH equation on a domain which is not a square (and hence we have 
no explicit kernel vectors and the multiplicity of BPs is not clear a priori) 
but which is $D_4$ invariant (such that in case of double BPs the amplitude 
equations still have the form \reff{sqae}). Essentially, here we transfer 
to the SH on a perturbed square some 
results from \cite{Craw91}, which explain why some double BPs break up while 
other stay double, and what primary bifurcations occur. 


\input{psqf2}

Thus, we consider \reff{swiho} on the domain $\Om_\del$ where we perturb 
the edges 
\hugast{ \Ga_1=\{(t,0)\},  \Ga_2=\{(2\pi,t)\}, 
\Ga_3=\{(2\pi{-}t,2\pi)\},  \Ga_4=\{(0,2\pi{-}t)\}} 
where $t\in[0,2\pi)$,  to  
\hugast{\Ga_1^\del=\{(t,\del\sin(\frac t 2))\}, 
\Ga_2^\del=\{(2\pi{-}\del\sin(\frac t 2),t)\}, 
\Ga_3^\del=\{(2\pi{-}t,2\pi{-}\sin(\frac t 2))\}, 
\Ga_4^\del=\{(\del\sin(\frac t 2),2\pi{-}t)\},}
see Fig.~\ref{shfpsq}(d) for the shape of $\Om_{0.35}$. 
In Fig.~\ref{shfpsq}(a) we recall the 'pure modes' 
\huga{\text{$\phi_{m,n}(x,y)=\cos(mx)\cos(ny)$, $n,m\in\N/2$,}}
at the first two branch points $\lam=0$ 
and $\lam=1/16$ on the (unperturbed) square $\Om=(0,2\pi)^2$ with Neumann BCs, 
where now we take the horizontal reflection 
$\ga_1:(x,y)\mapsto (\pi-x,y)$ and the diagonal reflection $\ga_2:(x,y)\mapsto(y,x)$ as the generators of $D_4$. Then $\ga_1\phi_{m,n}=(-1)^{2m}\phi_{m,n}$ 
and $\ga_{2}\phi_{m,n}=\phi_{m,n}$. 
In \cite{Craw91} it is explained that the 'mixed' modes 
$\phi_{m,n}^\pm=\phi_{m,n}\pm\phi_{n,m}$, see Fig.~\ref{shfpsq}(b), 
are more natural basis functions of the kernels. 
%The pure modes always fulfill $\ga_2\phi_{m,n}=\phi_{n,m}$, while 
These fulfill 
\huga{
\ga_2\phi_{m,n}^\pm=\pm\phi_{m,n}^\pm, 
} 
and 
\huga{
\ga_1\phi_{m,n}^\pm=(-1)^{2m}\times\left\{
\barr{ll}\phi_{m,n}^\pm&2(m+n)\text{ even (parity)}, \\
\phi_{m,n}^\mp&2(m+n)\text{ odd (parity)}.\earr\right.
} 
Using these symmetries, the effect of the perturbation $\del\sin(t/2)$ 
of the square is further analyzed in \cite{Craw91}. 
For odd parity, the perturbation analysis yields that the 
double eigenvalues stay double, with the simultaneous bifurcation 
of branches with pure and mixed mode symmetry. However, 
the even parity modes break 
into two BPs where only branches of mixed mode symmetry bifurcate,  
while the previously primary pure modes now become 
secondary bifurcation. Precisely this is illustrated in Fig.~\ref{shfpsq}(c,d) 
for the first two BPs, for $\del=0.35$. Additionally, the mixed mode 
branch {\tt mm1} now becomes transcritical as the hidden symmetry 
of a shift by half a period in $x$ or $y$ is lost, while all other branches 
remain pitchforks. 

\brem\label{hsymrem}
hidden symmetry enters twofold: 
\erem 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> schnakbcc.tex <==
 
\begin{figure}[h]
\bce 
\begin{tabular}{l}
{\small (a) BD on SC (sub)lattice, and example solutions from the {\tt rhombs} branch.}\\
\ig[width=0.17\textwidth]{pic/schnakpics/s3Dbd}\hs{2mm}
\raisebox{3mm}{\ig[width=0.18\textwidth]{pic/schnakpics/r-5}\hs{-0mm}
\ig[width=0.18\textwidth]{pic/schnakpics/r-10}\hs{-0mm}
%\ig[width=0.18\textwidth]{pic/schnakpics/r-15}\hs{-0mm}
\ig[width=0.18\textwidth]{pic/schnakpics/r-20}}\\
{\small (b) kernel vectors on the BCC (sub)lattice, and bifurcation direction for a BCC}\\[-1mm]
\ig[width=0.18\textwidth]{pic/schnakpics/bphi1}\hs{-0mm}
\ig[width=0.18\textwidth]{pic/schnakpics/bphi2}\hs{-0mm}
\ig[width=0.18\textwidth,height=31mm]{pic/schnakpics/bphi3}
\ig[width=0.18\textwidth]{pic/schnakpics/BCCtau3}\\
{\small (c) BD of BCCs and square-prisms on BCC lattice, and example solutions}\\[-0mm]
\hs{-5mm}\ig[width=0.2\textwidth,height=33mm]{pic/schnakpics/BCCbd}\hs{2mm}
\raisebox{2mm}{%\ig[width=0.18\textwidth]{pic/schnakpics/bcc3a-15}\hs{-0mm}
\ig[width=0.18\textwidth,height=35mm]{pic/schnakpics/bcc3a-25}\hs{-0mm}
\ig[width=0.18\textwidth]{pic/schnakpics/bcc3b-10}\hs{-0mm}
\ig[width=0.18\textwidth]{pic/schnakpics/bcc3t-20}}
\end{tabular}

\ece
\vs{-2mm}
   \caption{{\small {\red kommt weg.} 
\reff{tur1} on a SC lattice domain (a) and a BCC lattice domain (b,c), $\sig=0$. 
(a) On the SC, the kernel vectors are clean lamellas, the primary bifurcations are pitchforks, and the bifurcation directions are easily 
obtained from {\tt cswibra}; lamellas (red, stable up to $\lam\approx 2.52$), tubes (blue) and rhombs (magenta), 20 continuation steps for each, 
 $n_t=33000$ tetrahedra, see {\tt cmds3DSC.m} for details. 
(b) Left: Kernel vectors on the BCC domain look 
like distorted square prisms. Right: Bifurcation direction for a BCC solution, with $\al=(0.46,0.48,0.28)$. 
(c) BD of BCCs (red) and square prisms (blue), and three example solutions. The 'hot' 
BCC has already lost some of it's symmetry at pt10, while here the prisms continue 
without problems.  
$n_t=57024$ tetrahedra, see {\tt cmds3DBCC.m}. 
  \label{schnakf4}}}
\end{figure}

==> sh2df1.tex <==
\begin{figure}[ht]
\bce 
\begin{tabular}{llll}
(a) &&(b)&\\ 
\ig[width=0.22\textwidth]{pic/shsq/hexbd1}
&\hs{-6mm}\raisebox{25mm}{\begin{tabular}{l}
\ig[width=0.24\textwidth]{pic/shsq/h1}\\\ig[width=0.24\textwidth]{pic/shsq/pq}
\end{tabular}}
&\ig[width=0.22\textwidth]{pic/shsq/hexbd4}
&\hs{-6mm}\raisebox{25mm}{\begin{tabular}{l}
\ig[width=0.24\textwidth]{pic/shsq/h+}\\\ig[width=0.24\textwidth]{pic/shsq/h-}
\end{tabular}}
\end{tabular}

(c) bifurcation directions on stripe branch and example plots on 2ndary branches 
\ig[width=0.25\textwidth]{pic/shsq/stau1}\hs{-2mm}\ig[width=0.25\textwidth]{pic/shsq/sb1-5}\hs{-2mm}
\ig[width=0.25\textwidth]{pic/shsq/stau3}\hs{-2mm}\ig[width=0.25\textwidth]{pic/shsq/m1}

\ece 
\caption{{\small Bifurcation diagrams and example plots SH over a small rectangular domain permitting hex solutions, 
$\nu=0$ (a) and $\nu=1/2$ (b),(c). In (a) we only plot the primary branches, 
including the 'patchwork quilt' (pq). In (b) we also plot 
secondary branches from the stripes branch, and (c) shows the new tangent 
directions and example solutions on the branches bifurcating from the stripes. 
The first branch (black in (b)) connects the first two bifurcation points 
on the stripes in a loop and is not captured by the amplitude equations because it contains the wave vectors $k=(\pm \frac 1 4, \pm \frac{\sqrt{3}}2)$. 
The mixed modes (magenta branch in (b)) then bifurcate at the 
third bifurcation point, and, importantly, do not reconnect to the 
up hexagons. Instead they continue unstably to the right and compared 
to the up hexagons (which stay stable until at least $\lam=2$) contain 
additional critical modes, again not captured by the amplitude equations. \label{shf10}}}
\end{figure}


==> sh2df1b.tex <==
\begin{figure}[ht]
\bce 
\begin{tabular}{p{0.49\textwidth}p{0.49\textwidth}}
{\small (a) $\nu=0$ (cubic case), str and pq stable at bifurcation, hex unstable} &
{\small (b) $\nu=0.5$, transcritical bifurcation of hex, stripes initially unstable, stable after bif.~of mixed modes}\\[0mm]
\ig[width=0.22\textwidth]{pic/shsq/hexbd1}
\hs{-6mm}\raisebox{25mm}{\begin{tabular}{l}
\ig[width=0.24\textwidth]{pic/shsq/h1}\\\ig[width=0.24\textwidth]{pic/shsq/pq}
\end{tabular}}
&\ig[width=0.22\textwidth]{pic/shsq/hexbd4}
\hs{-6mm}\raisebox{25mm}{\begin{tabular}{l}
\ig[width=0.24\textwidth]{pic/shsq/h+}\\\ig[width=0.24\textwidth]{pic/shsq/h-}
\end{tabular}}
\end{tabular}
\ece 
\vs{-6mm}
\caption{{\small Example results from {\tt cmds2dhex.m}. Bifurcation diagrams and example plots SH over a small rectangular domain permitting hex solutions, 
$\nu=0$ (a) and $\nu=1/2$ (b). In (b) we plot $\min u_1$ for the 'gap' hexagons. The magenta branch corresponds to mixed modes. 
See  {\tt cmds2dhex.m} for details of the 
secondary branches from the stripes.  \label{shf10}}}
\end{figure}



==> shtf.tex <==
\begin{figure}[h]
\bce 
\begin{tabular}{lll}
{\small (a) solution from guess 1}&{\small (b) solution from guess 2}&{\small (c) evolution of guess 2}\\
\raisebox{20mm}{\begin{tabular}{l}
\ig[width=0.3\textwidth]{pic/sh4/igs1}\\[-6mm]
\ig[width=0.3\textwidth]{pic/sh4/sol1}
\end{tabular}}&
\raisebox{20mm}{\begin{tabular}{l}
\ig[width=0.3\textwidth]{pic/sh4/igs2}\\[-6mm]
\ig[width=0.3\textwidth]{pic/sh4/sol2}
\end{tabular}}&
\ig[width=0.2\textwidth]{pic/sh4/ts}
\end{tabular}
\ece 
\vs{-6mm}
\caption{{\small Obtaining solutions from guesses, if necessary inluding time-integration ... \label{shtf}}}
\end{figure}


